Newton-type Alternating Minimization Algorithm for Convex Optimization

We propose NAMA (Newton-type Alternating Minimization Algorithm) for solving structured nonsmooth convex optimization problems where the sum of two functions is to be minimized, one being strongly convex and the other composed with a linear mapping. The proposed algorithm is a line-search method over a continuous, real-valued, exact penalty function for the corresponding dual problem, which is computed by evaluating the augmented Lagrangian at the primal points obtained by alternating minimizations. As a consequence, NAMA relies on exactly the same computations as the classical alternating minimization algorithm (AMA), also known as the dual proximal gradient method. Under standard assumptions the proposed algorithm possesses strong convergence properties, while under mild additional assumptions the asymptotic convergence is superlinear, provided that the search directions are chosen according to quasi-Newton formulas. Due to its simplicity, the proposed method is well suited for embedded applications and large-scale problems. Experiments show that using limited-memory directions in NAMA greatly improves the convergence speed over AMA and its accelerated variant.

==> TeX/Algs/NAMA_fixed.tex <==
\begin{algorithmic}[1]
	\Require{
		\(y^0\in\R^m\),
		\(\gamma \in (0,\mu_f / \|A\|^2) \),
		\(\beta\in(0,1)\)%
	}%
	%
	\Initialize{%
		\(k = 0\)%
	}%
%	\label{step:AMLS1_init}
	%
	\STATE\label{step:AMLS1_altmin}
		\(x^k = \argmin_{x} \set{f(x) + \innprod{y^k}{Ax}}\),~
		% \(x^k = \argmin_{x} \Ell(x, y^k)\),~
		\(z^k = \argmin_{z} \Ell_\gamma(x^k, z, y^k)\)%,~
		% \(z^k = \argmin_{z} \Ell_{\gamma}(x^k, z, y^k)\),~
		% \(z^k = \prox_{\gamma^{-1} g}(\gamma^{-1}y^k+Ax^k)\),~
		% \(r^k = z^k - Ax^k\)%
	%
	\STATE\label{step:AMLS1_direction}
		Choose a direction \(d^k\in\R^m\)
	%
	\STATE\label{step:AMLS1_linesearch}
		Find the largest \(\tau_k=\beta^{m_k}, m_k\in\N,\) such that
		\begin{equation}\label{eq:AMLS_ascent}
			\Ell_{\gamma}(\lspoint x^k, \lspoint z^k, \lspoint y^k) \geq \Ell_{\gamma}(x^k, z^k, y^k),
			\quad\text{where}\quad
			\begin{cases}[r@{{}={}}l]
				\lspoint y^k & y^k + \tau_k d^k + \gamma (1-\tau_k) (Ax^k-z^k)\\
				\lspoint x^k & \argmin_{x} \set{f(x) + \innprod{\tilde y^k}{Ax}}\\
				% \lspoint x^k & \argmin_{x} \Ell(x, \lspoint y^k)\\
				\lspoint z^k & \argmin_{z} \Ell_\gamma(\lspoint x^k, z, \lspoint y^k)
				% \lspoint z^k & \argmin_{z} \Ell_{\gamma}(\lspoint x^k, z, \lspoint y^k)
				% \lspoint z^k & \prox_{\gamma^{-1} g}(\gamma^{-1}\lspoint y^k+A \lspoint x^k)%\\
%				\argmin_{z\in\R^n} \Ell_{\gamma}(\lspoint x^k, z, \lspoint y^k)
			\end{cases}
		\end{equation}
%		where~~
%		\(\lspoint y^{k} = y^k + \tau_k d^k + (1-\tau_k) \gamma r^k\)
%
%		\noindent
%		and~
%		\(\lspoint x^k = \argmin_{x} \Ell(x, \lspoint y^k)\),~
%		\(\lspoint z^k = \prox_{\gamma^{-1} g}(\gamma^{-1}\lspoint y^k+A \lspoint x^k)\)% \argmin_{z\in\R^n} \Ell_{\gamma}(\lspoint x^k, z, \lspoint y^k)
	%
	\STATE\label{step:AMLS1_global}
		\(y^{k+1} = \lspoint y^k + \gamma (A\lspoint x^k - \lspoint z^k)\),
		\(k = k+1\),
		go to step \ref{step:AMLS1_altmin}
\end{algorithmic}


==> TeX/Algs/OLD_AMLS1_adaptive.tex <==
\begin{algorithmic}[1]
	\Require
		\(y^0\in\R^m\),
		\(\gamma_0 > 0\),
		\(\alpha,\beta,\delta\in(0,1)\),
		\(\sigma > 1\)%
	%
	\Initialize
		\(k\gets 0\),
		\(x^0 \gets \argmin_{x} \Ell(x, y^0)\),
		\(z^0 \gets \argmin_{z} \Ell(x^0, z, y^0)\)%
%	\label{step:AMLS1_init}
	%
	\STATE\label{step:AMLS1_ybar}
		\(\bar y^k \gets y^k + \gamma_k(Ax^k+Bz^k-b)\)%
	%
	\STATE\label{step:AMLS1_xbar}
		\(\bar x^k\gets\argmin_x\Ell_0(x,\bar y^k)\)%
	%
	\STATE\label{step:AMLS1_gamma}
		{\bf if}
		\(f(x^k) > f(\bar x^k) - \innprod{\trans{A} \bar y^k}{x^k - \bar x^k} + \tfrac{\alpha\gamma_k}{2}\|Ax^k+Bz^k-b\|^2\)
		{\bf then}
		\[
			\gamma_k \gets \delta\gamma_k,~
			z^k\gets\argmin_{z\in\R^n}\Ell_{\gamma_k}(x^k,z,y^k),~
			\text{go to step \ref{step:AMLS1_ybar}}
		\]
	%
	\STATE\label{step:AMLS1_direction}
		Choose a direction \(d^k\in\R^m\)
	%
	\STATE\label{step:AMLS1_linesearch}
		Find the largest \(\tau_k=\beta^{m_k}, m_k\in\N,\) such that if \(y^{k+1} \gets \bar y^k + \tau_k d^k\)
		and
		\[
			x^{k+1} \gets \argmin_{x\in\R^m} \Ell(x, y^{k+1}),~
			z^{k+1} \gets \argmin_{z\in\R^n} \Ell_{\gamma_k}(x^{k+1}, z, y^{k+1})
		\]
		then
		\(\Ell_{\gamma_k}(x^{k+1}, z^{k+1}, y^{k+1}) \geq \Ell_{\gamma_k}(x^k, z^k, y^k) + \tfrac{(1-\alpha)\gamma_k}{2\sigma}\|Ax^k + Bz^k - b\|^2\)
	%
	\STATE
		\(\gamma_{k+1} \gets \gamma_k\),
		\(k\gets k+1\),
		go to step \ref{step:AMLS1_ybar}
\end{algorithmic}


==> TeX/Algs/OLD_AMLS1_fixed.tex <==
\begin{algorithmic}[1]
	\Require
		\(y^0\in\R^m\),
		\(\gamma = \alpha/\lip\nabla\psi_1\),
		\(\alpha,\beta\in(0,1)\),
		\(\sigma > 1\)%
	%
	\Initialize%\label{step:AMLS1_fixed_init}
		\(k\gets 0\),
		\(x^0 \gets \argmin_{x} \Ell(x, y^0)\),
		\(z^0 \gets \argmin_{z} \Ell(x^0, z, y^0)\)%
	%
	\STATE\label{step:AMLS1_fixed_ybar}
		\(\bar y^k \gets y^k + \gamma(Ax^k+Bz^k-b)\)%
	%
	\STATE\label{step:AMLS1_fixed_direction}
		Choose a direction \(d^k\in\R^m\)%
	%
	\STATE\label{step:AMLS1_fixed_linesearch}
		Find the largest \(\tau_k=\beta^{m_k}, m_k\in\N,\) such that if \(y^{k+1} \gets \bar y^k + \tau_k d^k\)
		and
		\[
			x^{k+1} \gets \argmin_{x\in\R^m} \Ell(x, y^{k+1}),~
			z^{k+1} \gets \argmin_{z\in\R^n} \Ell_{\gamma}(x^{k+1}, z, y^{k+1})
		\]
		then
		\(\Ell_{\gamma}(x^{k+1}, z^{k+1}, y^{k+1}) \geq \Ell_{\gamma}(x^k, z^k, y^k) + \tfrac{(1-\alpha)\gamma}{2\sigma}\|Ax^k + Bz^k - b\|^2\)
	%
	\STATE
		\(k\gets k+1\),
		go to step \ref{step:AMLS1_fixed_ybar}
\end{algorithmic}


==> TeX/Algs/OLD_AMLS2_adaptive.tex <==
\begin{algorithmic}[1]
	\Require
		\(y^0\in\R^m\),
		\(\gamma_0 > 0\),
		\(\alpha,\beta,\delta\in(0,1)\),
		\(\sigma > 1\)%
	%
	\Initialize
		\(k\gets 0\)%
%	\label{step:AMLS1_init}
	%
	\STATE\label{step:AMLS1_altmin}
		\(x^k \gets \argmin_{x} \Ell(x, y^k)\),
		\(z^k \gets \argmin_{z} \Ell_{\gamma_k}(x^k, z, y^k)\),
		\(r^k \gets Ax^k+Bz^k-b\)%
	%
	\STATE\label{step:AMLS1_xbar}
		\(\bar y^k \gets y^k + \gamma_k r^k\),
		\(\bar x^k\gets\argmin_x\Ell_0(x, \bar y^k)\)%
	%
	\STATE\label{step:AMLS1_gamma} 
		{\bf if}
		\(f(x^k) > f(\bar x^k) - \innprod{\trans{A} \bar y^k}{x^k - \bar x^k} + \tfrac{\alpha\gamma_k}{2}\|r^k\|^2\)
		{\bf then}
		\[
			\gamma_k \gets \delta\gamma_k,~
			z^k\gets\argmin_{z\in\R^n}\Ell_{\gamma_k}(x^k,z,y^k),~
			r^k \gets Ax^k+Bz^k-b,~
			\text{go to \ref{step:AMLS1_xbar}}
		\]
	%
	\STATE\label{step:AMLS1_direction}
		Choose a direction \(d^k\in\R^m\)
	%
	\STATE\label{step:AMLS1_linesearch}
		Find largest \(\tau_k=\beta^{m_k}, m_k\in\N,\) s.t. \(\Ell_{\gamma_k}(\lspoint x^k, \lspoint z^k, \lspoint y^k) \geq \Ell_{\gamma_k}(x^k, z^k, y^k)\) where
		\[\lspoint y^{k} \gets y^k + \tau_k d^k + (1-\tau_k) \gamma_k r^k\]
		and
		\(
			\lspoint x^k \gets \argmin_{x\in\R^m} \Ell(x, \lspoint y^k),~
			\lspoint z^k \gets \argmin_{z\in\R^n} \Ell_{\gamma_k}(\lspoint x^k, z, \lspoint y^k)
		\)
	%
	\STATE
		\(y^{k+1} \gets \lspoint y^k + \gamma_k (A\lspoint x^k+B\lspoint z^k-b)\),
		\(\gamma_{k+1} \gets \gamma_k\),
		\(k\gets k+1\),
		go to \ref{step:AMLS1_altmin}
\end{algorithmic}


==> TeX/Text/FBE.tex <==
The fundamental tool enabling fast convergence of \Cref{alg:NAMA} is the \emph{forward-backward envelope} function associated with \eqref{eq:DualProblem}:
we now recall its definition and fundamental properties, and then illustrate how they are related to \eqref{eq:Problem}.
The following definition corresponds to \cite[Def. 2.1]{stella2016forward}.

\begin{defin}\label{def:FBE}
The \DEF{forward-backward envelope} function (FBE) associated with the problem of minimizing \(\psi(y) = \conj f(-\trans{A}y) + \conj g(y)\) is given by
\EXCEPT{ieee}{%
	\begin{equation}\label{eq:FBE}
			\psi_\gamma(y)
		{}={}
			\inf_{w\in\R^m}\set{
				\tf(y) + \innprod{\nabla\tf(y)}{w-y} + \conj g(w) + \tfrac{1}{2\gamma}\|w-y\|^2
			}.
	\end{equation}
}%
\ONLY{ieee}{%
	\begin{align}
	\nonumber
			\psi_\gamma(y)
		{}={}
			\inf_{w\in\R^m}\Bigl\{
		&
				\hphantom{{}+{}}
				\tf(y) + \innprod{\nabla\tf(y)}{w-y}
		\\[-5pt]
		&
			\fillwidthof[l]{
				\hphantom{{}+{}}
				\tf(y) + \innprod{\nabla\tf(y)}{w-y}
			}{
				{}+\conj g(w) + \tfrac{1}{2\gamma}\|w-y\|^2
			}
			\Bigr\}.
	\label{eq:FBE}
	\end{align}
}%
where \(\tf=\conj f\circ(-\trans A)\) and \(\gamma>0\) is a given parameter.
\end{defin}

The FBE is a real-valued function, as opposed to extended real-valued as it is the case for \(\psi\), and can be equivalently expressed in terms of the Moreau envelope of \(\conj g\) as follows
\EXCEPT{ieee}{%
	\begin{align}
	\label{eq:EquivFBE}
		\psi_\gamma(y)
	{}={} &
		\conj f(-\trans Ay)
		{}-{}
		\tfrac{\gamma}{2}\|A\nabla\conj f(-\trans Ay)\|^2
		{}+{}
		(\conj g)^{\gamma}(y+\gamma A\nabla\conj f(-\trans Ay))
	\\
	\label{eq:FBEexp}
	{}={} &
		\conj f(-\trans Ay)
		{}+{}
		\conj g(T_{\gamma}(y))
		{}+{}
		\gamma\innprod{A\nabla \conj f(-\trans Ay)}{R_\gamma(y)}
		{}+{}
		\tfrac{\gamma}{2}\|R_\gamma(y)\|^2,
	\end{align}
}%
\ONLY{ieee}{%
	\begin{align}
	\nonumber
		\psi_\gamma(y)
	{}={} &
		\hphantom{{}+{}}
		\conj f(-\trans Ay)
		{}-{}
		\tfrac{\gamma}{2}\|A\nabla\conj f(-\trans Ay)\|^2
	\\
	\label{eq:EquivFBE}
	&
		{}+{}
		(\conj g)^{\gamma}(y+\gamma A\nabla\conj f(-\trans Ay))
	\\
	\nonumber
	{}={} &
		\hphantom{{}+{}}
		\conj f(-\trans Ay)
		{}+{}
		\conj g(T_{\gamma}(y))
	\\
	\label{eq:FBEexp}
	&
		{}+{}
		\gamma\innprod{A\nabla \conj f(-\trans Ay)}{R_\gamma(y)}
		{}+{}
		\tfrac{\gamma}{2}\|R_\gamma(y)\|^2,
	\end{align}
}%
see \cite{patrinos2013proximal}.
However, in the setting of the present paper, \(\psi_\gamma\) has a very simple interpretation in terms of the augmented Lagrangian associated with problem \eqref{eq:Problem}, as we now show.

\begin{thm}\label{thm:AME}
For \(y\in\R^m\) and \(\gamma>0\), let \(x(y)\) and \(z_\gamma(y)\) be as in \eqref{eq:AMM}.
Then,
\begin{equation}\label{eq:AMEvsFBE}
	\psi_\gamma(y) = -\Ell_\gamma(x(y),z_\gamma(y),y).
\end{equation}
\begin{proof}
Applying \eqref{eq:ConjSubgr} to \(f\) we see that for all \(y\in\R^m\)
\begin{align}
\label{eq:PrimalGradPsi1}
	\nabla \conj f(-\trans{A} y)
{}={} &
	\argmin_{x\in\R^n}\set{f(x) + \innprod{y}{Ax}}
{}={}
	x(y),
\\
%	\nabla\tf(y)
%{}={} &
%	{-A\nabla \conj f(-\trans{A} y)}
%	{}={}
%	-Ax(y),
%\\
\label{eq:PrimalPsi1}
	\conj f(-\trans{A} y)
{}={} &
	-f(x(y))-\innprod{y}{Ax(y)}.
\end{align}
Using \eqref{eq:PrimalGradPsi1} and \eqref{eq:PrimalPsi1} we can rewrite the FBE as
\EXCEPT{ieee}{%
	\begin{align}
		\psi_\gamma(y)
	{}={}&
		{\inf}_{u\in\R^m}
		\set{
			\conj f(-\trans{A}y)-\innprod{A\nabla\conj f(-\trans{A}y)}{u-y}
			+\conj g(u)+\tfrac{1}{2\gamma}\|u-y\|^2
		}\nonumber
	\\
	{}={}&
		-f(x(y)) + {\inf}_{u\in\R^m}\set{
			\conj g(u)-\innprod{Ax(y)}{u}+\tfrac{1}{2\gamma}\|u-y\|^2
		}.\label{eq:AugmentedLagrangianDual}
	\end{align}
}%
\ONLY{ieee}{%
	\begin{align}
		\psi_\gamma(y)
	{}={}&
		\inf_{u\in\R^m}\Bigl\{
			\hphantom{{}+{}}
			\conj f(-\trans{A}y)-\innprod{A\nabla\conj f(-\trans{A}y)}{u-y}\nonumber
	\\[-8pt]
	&
		\hphantom{\inf_{u\in\R^m}\Bigl\{}
			{}+\conj g(u)+\tfrac{1}{2\gamma}\|u-y\|^2
		\Bigr\}\nonumber
	\\
	{}={}&
		\inf_{u\in\R^m}\Bigl\{
			\conj g(u)-\innprod{Ax(y)}{u}+\tfrac{1}{2\gamma}\|u-y\|^2
		\Bigr\}\label{eq:AugmentedLagrangianDual}
	\\
		{}& -f(x(y)).\nonumber
	\end{align}
}%
Due to \cref{ass:Strong} and \cite[Thm. 11.42]{rockafellar2011variational}, \cite[Cor. 31.2.1]{rockafellar1997convex}, strong duality holds for the \(\inf\) in \eqref{eq:AugmentedLagrangianDual}. Therefore
\begin{align*}
	& \phantom{-} \inf_{u\in\R^m}\Bigl\{
		\conj g(u)-\innprod{Ax(y)}{u}+\tfrac{1}{2\gamma}\|u-y\|^2
	\Bigr\} \\
	= & - \inf_{z\in\R^m}\set{g(z)+\innprod{y}{Ax(y) - z}+\tfrac{\gamma}{2}\|Ax(y)-z\|^2},
\end{align*}
which substituted in \eqref{eq:AugmentedLagrangianDual} yields
\[\psi_\gamma(y) = -\Ell_\gamma(x(y),z_\gamma(y),y),\]
concluding the proof.
% substituting it with its dual problem we obtain
% \EXCEPT{ieee}{%
% 	\begin{align*}
% 		\psi_\gamma(y)
% 	{}={}&
% 		-f(x(y)) - {\inf}_{z\in\R^m}\set{g(z)+\innprod{y}{Ax(y) - z}+\tfrac{\gamma}{2}\|Ax(y)-z\|^2} \\
% 	{}={}& -\Ell_\gamma(x(y),z_\gamma(y),y)
% 	\end{align*}
% }%
% \ONLY{ieee}{%
% 	\begin{align*}
% 		\psi_\gamma(y)
% 	{}=&
% 		-\inf_{z\in\R^m}\!\set{g(z)+\innprod{y}{Ax(y) - z}+\tfrac{\gamma}{2}\|Ax(y)-z\|^2}
% 	\\
% 	&
% 		-f(x(y))
% 	\\
% 	{}={}& -\Ell_\gamma(x(y),z_\gamma(y),y)
% 	\end{align*}
% }%
% which concludes the proof.
\end{proof}
\end{thm}

The FBE enjoys several favorable properties, some of which we now summarize.
For any \(\gamma>0\) the FBE \(\psi_\gamma\) is (strictly) continuous over \(\R^m\), whereas if \(\gamma\) is small enough it shares with \(\psi\) the infimum value and the set of minimizers.
As a consequence, solving \eqref{eq:DualProblem} is equivalent to minimizing \(\psi_\gamma\) when \(\gamma\) is small enough.
These properties are listed in the next result.
\begin{thm}\label{thm:FBEbounds}
For any \(\gamma>0\), \(\psi_\gamma\) is a strictly continuous function on \(\R^m\) satisfying
\begin{enumerate}
	\item\label{it:FBEleq}
		\(
			\psi_\gamma(y)
		{}\leq{}
			\psi(y) - \tfrac\gamma 2\|R_\gamma(y)\|^2
		\);
	\item\label{it:FBEgeqGlobal}
		\(
			\psi(T_\gamma(y))
		{}\leq{}
			\psi_\gamma(y)
			{}-{}
			\gamma\tfrac{1-\gamma \mu_f^{-1}\|A\|^2}{2}
			\|R_\gamma(y)\|^2
		\).
\end{enumerate}
for any \(y\in\R^m\).
In particular, if \(\gamma<\nicefrac{\mu_f}{\|A\|^2}\), then the following also holds
\begin{enumerate}[resume]
	\item\label{it:EquivFBE}
		\(\inf\psi=\inf\psi_\gamma\)
		and
		\(\argmin\psi=\argmin\psi_\gamma\).
\end{enumerate}
\begin{proof}
Let \(\tf=\conj f\circ(-\trans A)\) and \(L_\tf=\nicefrac{\|A\|^2}{\mu_f}\).
As shown in \cref{rem:Basic}, both \((\conj g)^\gamma\) and \(\nabla\tf\) are strictly continuous, and therefore so is \(\psi_\gamma\), as it is apparent from the expression \eqref{eq:EquivFBE}.

Using \cref{lem:TwoPointsIneq} with \(w = y\) yields \eqref{it:FBEleq}.

To see \ref{it:FBEgeqGlobal}, observe that
\EXCEPT{ieee}{%
	\begin{align*}
		\psi_\gamma(y)
	{}={} &
		\tf(y) + \gamma\innprod{\nabla\tf(y)}{R_\gamma(y)} + \conj g(T_{\gamma}(y)) + \tfrac{\gamma}{2}\|R_\gamma(y)\|^2
	\\
	{}\geq{} &
		\tf(T_\gamma(y)) + \conj g(T_{\gamma}(y)) - \tfrac{L_\tf}{2}\|T_{\gamma}(y)-y\|^2 + \tfrac{\gamma}{2}\|R_\gamma(x)\|^2.
	\end{align*}
}%
\ONLY{ieee}{%
	\begin{align*}
		\psi_\gamma(y)
	{}={} &
		\tf(y) + \gamma\innprod{\nabla\tf(y)}{\!\!R_\gamma(y)} + \conj g\!(T_{\gamma}(y)) {+{}} \tfrac{\gamma}{2}\|R_\gamma(y)\|^2
	\\
	{}\geq{} &
		\hphantom{{}+{}}
		\tf(T_\gamma(y)) + \conj g(T_{\gamma}(y)) - \tfrac{L_\tf}{2}\|T_{\gamma}(y)-y\|^2
	\\
	&
		{}+\tfrac{\gamma}{2}\|R_\gamma(y)\|^2.
	\end{align*}
}%
where the inequality is due to \eqref{Eq:DescentLemma}.

Combining the two inequalities, \ref{it:EquivFBE} easily follows.
\end{proof}
\end{thm}


==> TeX/Text/LemmaConvergenceIterates.tex <==
\begin{lem}\label{lem:dual2primal}
For any $y\in\R^m$ it holds that
%\begin{enumerate}
%\item
\(
	\tfrac{\mu_f}{2}\|x(y)-x_\star\|^2 \leq \psi(y) - \inf\psi
\).
%\end{enumerate}
%If moreover $\gamma\in(0, \mu_f/\|A\|^2]$ then
%\begin{enumerate}
%\setcounter{enumi}{1}
%\item\label{eq:dualsubopt2Bz}
%	\(\tfrac{\gamma}{2}\|Ax_\star + Bz_\gamma(y) - b\|^2 \leq \psi(y) - \inf\psi,\)
%\item\label{eq:dualsubopt2res}
%	\(\tfrac{\gamma}{2}\|Ax(y)+Bz_\gamma(y)-b\|^2 \leq \psi(y) - \inf\psi.\)
%\end{enumerate}

\begin{proof}
%We can assume that \(y\in\R^m\) is dual feasible, otherwise the bounds hold trivially.
%Let us denote for brevity of notation \(x = x(y) = \argmin\set{f(\cdot) + \innprod{y}{A\cdot}}\).
%Therefore \(-\trans{A}y \in \partial f(x)\), and using strong convexity of \(f\) we can write
%\begin{subequations}\label{eq:twoineq}\begin{align}
%	f(x) - \innprod{\trans{A}y}{x_\star - x} + \tfrac{\mu_f}{2}\|x_\star-x\|^2
%{}\leq{}&
%	f(x_\star),
%\end{align}\end{subequations}
We can assume that \(y\in\R^m\) is dual feasible, otherwise the bound holds trivially.
Since \(x(y) = \argmin\set{f(\cdot) + \innprod{y}{A\cdot}}\) and \(f\) is strongly convex, we have
\begin{align*}
	\inf\set{f(\cdot) + \innprod{y}{A\cdot}} + \tfrac{\mu_f}{2}\|x(y)-x_\star\|^2
{}\leq{}&
	f(x_\star) + \innprod{y}{Ax_\star},
\\
	\inf\{g(\cdot) - \innprod{y}{\cdot}\}
{}\leq{}&
	g(A x_\star) - \innprod{y}{A x_\star}.
\end{align*}
%where \(z_\star\in Z_\star\).
The $\inf$ in second inequality is finite, since \(y\) is dual feasible by assumption.
%Recall that \(\psi(y) = -\inf_{x,z}\Ell_0(x, z, y)\), and note that \(Ax_\star+Bz_\star = b\). Therefore,
Summing the two inequalities and subtracting \(\innprod{y}{b}\) to both sides, one obtains
\[
	-\psi(y) + \tfrac{\mu_f}{2}\|x_\star-x(y)\|^2 \leq f(x_\star) + g(z_\star),
\]
and the proof follows by strong duality.
%Let's now indicate \(x = x(y)\) and \(z = z_\gamma(y)\) for brevity.
%It holds
%\begin{align}
%\psi(y) + \Ell_\gamma(x,z,y) &= \psi(y)+\Ell_0(x,z,y) + \tfrac{\gamma}{2}\|Ax+Bz-b\|^2\nonumber\\
%    & \geq \tfrac{\gamma}{2}\|Ax+Bz-b\|^2,\label{eq:ineq3}
%\end{align}
%where the inequality follows since
%\(\psi(y) = -\inf_{x,z}\Ell_0(x, z, y)\).
%Now, observe that
%\begin{align}
%\Ell_\gamma(x,z_\star,y)-\Ell_\gamma(x,z,y) {}={}&
%	g(z_\star)-g(z)+\innprod{\trans{B} y}{z_\star-z} \nonumber \\
%		&+ \tfrac{\gamma}{2}\|Ax+Bz_\star-b\|^2	- \tfrac{\gamma}{2}\|Ax+Bz-b\|^2.\label{eq:sonasega}
%\end{align}
%The optimality condition of the problem defining \(z_\gamma(y)\) reads
%\[ -\trans{B} (y + \gamma (Ax+Bz-b)) \in \partial g(z),\]
%therefore we can use subgradient inequality on \(g\) to rewrite \eqref{eq:sonasega} as
%\begin{align}
%\Ell_\gamma(x,z_\star,y)-\Ell_\gamma(x,z,y)
%	{}\geq{}& -\gamma\innprod{\trans{B}(Ax+Bz-b)}{z_\star-z} \nonumber \\
%	& + \tfrac{\gamma}{2}\|Ax+Bz_\star-b\|^2	- \tfrac{\gamma}{2}\|Ax+Bz-b\|^2 \nonumber \\
%	{}={}& \tfrac{\gamma}{2}\|Bz_\star\|^2 - \tfrac{\gamma}{2}\|Bz\|^2 -\gamma\innprod{Bz}{B(z_\star-z)} \nonumber \\
%	{}={}& \tfrac{\gamma}{2}\|B(z_\star-z)\|^2 \nonumber \\
%	{}={}& \tfrac{\gamma}{2}\|Ax_\star + Bz - b\|^2. \label{eq:ineq2}
%\end{align}
%Finally, we have what follows:
%\begin{align*}
%-\inf\psi - \Ell_\gamma(x,z_\star,y) &= f(x_\star) + g(z_\star) - f(x) - g(z_\star)\\
%    & \phantom{=} - \innprod{y}{Ax+Bz_\star-b} - \tfrac{\gamma}{2}\|Ax+Bz_\star-b\|^2\\
%    &= f(x_\star) - f(x) + \innprod{\trans{A} y}{x_\star-x} - \tfrac{\gamma}{2}\|A(x_\star-x)\|^2\\
%    &\geq \tfrac{\mu_f}{2}\|x_\star-x\|^2-\tfrac{\gamma}{2}\|A(x_\star-x)\|^2,
%\end{align*}
%where the first equality follows from strong duality, the second holds since \(x_\star\) and \(z_\star\) are primal feasible and the inequality follows from strong convexity of \(f\) and the fact that \(x\) minimizes \(f+\innprod{\trans{A} y}{\cdot}\).
%So
%\begin{equation}\label{eq:ineq1}
%-\inf\psi - \Ell_\gamma(x,z_\star,y) \geq \tfrac{\mu_f-\gamma\|A\|^2}{2}\|x_\star-x\|^2,
%\end{equation}
%where the right-hand side is nonnegative whenever \(\gamma \leq \mu_f/\|A\|^2\).
%Adding \eqref{eq:ineq3}, \eqref{eq:ineq2}, \eqref{eq:ineq1} we obtain \cref{eq:dualsubopt2Bz}
%and \cref{eq:dualsubopt2res}.
\end{proof}
\end{lem}


==> TeX/Text/Simulations/Hankel.tex <==
We consider the problem of estimating the impulse response coefficients and the order of a MIMO, linear time-invariant (LTI), discrete-time system given \(2M\) uniformly spaced, noisy samples of the frequency response \cite{mckelvey1996subspace}.

Letting \(n_u, n_y\) be the number of inputs and outputs to the system, we follow the procedure described in \cite{plessen2015optimization} and solve the nuclear norm regularized least-squares problem
\begin{equation}\label{eq:HankelRankMin}
	\minimize_{x\in\R^{n_y \times 2Mn_u}}\ p(x) = \tfrac12\|x - b\|_F^2 + \mu\|H(x)\|_*,
\end{equation}
where \(b\in\R^{n_y \times 2Mn_u}\) contains noisy impulse response estimates and \(\|\cdot\|_* = \sum_i \sigma_i(\cdot)\) where \(\sigma_i\) is the \(i\)-th singular value of the matrix argument. Furthermore, partitioning the variable \(x\) as
\[x = \begin{pmatrix} x_1 &\ x_2 &\ \ldots &\ x_{2M} \end{pmatrix}, \quad x_i\in\R^{n_y\times n_u},\ i = 1,\ldots,2M,\]
the \emph{Hankel operator} \(H\) is defined as
\[
	H(x) = \begin{bmatrix}
		x_1 &\ x_2 &\ \cdots &\ x_q \\
		x_2 &\ x_3 &\ \cdots &\ x_{q+1} \\
		\vdots &\ \vdots &\ \ddots &\ \vdots \\
		x_p &\ x_{p+1} &\ \cdots &\ x_{p+q-1}
	\end{bmatrix} \in \R^{pn_y\times qn_u},
\]
for integer parameters \(p, q\) satisfying \(p+q-1 = 2M\). The nuclear norm term in \eqref{eq:HankelRankMin} is known to enforce sparsity in \(H(x_\star)\) at the singular values level, therefore parameter \(\mu>0\) allows to modulate between a good least-squares fit at the solution and a low rank \(H(x_\star)\).

To perform our experiments we have considered \(n_u = n_y = 1\) and \(M=100\), and the data \(b\) was obtained with a randomly generated LTI with \(n_x = 6\) and additive Gaussian noise with variance \(0.01\).

We compared \eqref{alg:NAMA} to fast AMA, which is thoroughly discussed in \cite{plessen2015optimization} in application to problem \eqref{eq:HankelRankMin}. Note that in this case the convexity parameter of \(f\) is \(\mu_f=1\), while \(\|H\| = \min\set{p,q}\). We used as termination criterion for the algorithms \(|p(x^k) + \psi(y^k)|/(1+|\psi(y^k)|) \leq \epsilon_{\mathrm{tol}}\), \ie, a tolerance on the relative duality gap, computed every \(10\) iterations.

From \Cref{fig:HankelConvergence} it is apparent how \algacronym\ accelerates the convergence of the classical alternatint minimization algorithms, exhibiting fast linear convergence when (limited memory) quasi-Newton directions are used. In \Cref{fig:HankelSV}, for the same setting, the distribution of the largest singular values of the computed \(H(x_\star)\) is shown in the case where \(\epsilon_{\mathrm{tol}} = 10^{-4}, 10^{-8}\): by restricting the tolerance model \eqref{eq:HankelRankMin} is able to much better identify the order of the system. \Cref{fig:HankelWarmStart} shows the performance of the algorithms in computing a full regularization path with \(\epsilon_{\mathrm{tol}} = 10^{-8}\), for increasing values of the parameter \(\mu \in (0.003, 0.3)\) and warm-starting each problem with the solution to the previous one.

\begin{figure}
\input{TeX/Tikz/Hankel_FPR_convergence}
\caption{Convergence of the fixed point residual \(\|R_\gamma(y^k)\| = \|H(x^k) - z^k\|\) in the considered algorithms.}\label{fig:HankelConvergence}
\end{figure}

\begin{figure}
\input{TeX/Tikz/Hankel_SV_tol_1e-4}
\input{TeX/Tikz/Hankel_SV_tol_1e-8}
\caption{Distribution of the \(20\) largest singular values at the solutions computed by different algorithms, in the case of \(\mu = 0.02\). Left: \(\epsilon_{\mathrm{tol}} = 10^{-4}\). Right: \(\epsilon_{\mathrm{tol}} = 10^{-8}\).}\label{fig:HankelSV}
\end{figure}

\begin{figure}
\input{TeX/Tikz/Hankel_SISO_mu_vs_cputime}
\caption{Performance of the methods in the case of a SISO system. Problem \eqref{eq:HankelRankMin} was solved with \(100\) increasing values of the parameter \(\mu\) logarithmically spaced in \([0.003, 0.3]\), warm-starting each problem by initializing \(y^0\) to the solution of the previous one.}\label{fig:HankelWarmStart}
\end{figure}


%Let the state-space model of the system be
%\begin{subequations}\label{eq:LTI}\begin{align}
%	x(k+1) &= Ax(k) + Bu(k), \\
%	y(k) &= Cx(k) + Du(k),
%\end{align}\end{subequations}
%with \(x\in\R^{n_x}\), \(u\in\R^{n_u}\), \(y\in\R^{n_y}\), and matrices \(A, B, C, D\) of the appropriate dimension. The frequency response for \eqref{eq:LTI} is given by
%\[G(e^{j\omega}) = C(e^{j\omega}I-A)^{-1}B + D\]

%We consider the problem
%\begin{equation}
%	\minimize_{Y \in \R^{p\times q(N+1)}}\ \tfrac{1}{2}\|Y-W\|_F^2 + \|H_r(Y)Q\|_*.
%\end{equation}
%Here \(H_r:\R^{p\times q(N+1)} \to \R^{pr\times q(N-r+1)}\) is the Hankel matrix operator defined as
%\[ H_r(Y) =
%	\begin{pmatrix}
%		Y_0 &\ Y_1 &\ \cdots &\ Y_{N-r} \\
%		Y_1 &\ Y_2 &\ \cdots &\ Y_{N-r+1} \\
%		\vdots &\ \vdots &\ \ddots &\ \vdots \\
%		Y_r &\ Y_{r+1} &\ \cdots &\ Y_N
%	\end{pmatrix},
%\]
%where \(Y_i\in\R^{p\times q}\) are blocks of \(Y = \begin{pmatrix} Y_0 &\ Y_1 &\ \ldots &\ Y_{N} \end{pmatrix}\).
%Matrix \(Q\) is orthogonal, while \(\|\cdot\|_F\) and \(\|\cdot\|_*\) indicate the Frobenius and nuclear norm respectively.
%
%This problem arises in the field of system identification, see for example \cite{liu2010interior,fazel2013hankel}, where the goal is to identify a linear time-invariant dynamical system from input and output measurements:
%in this case \(U = \begin{pmatrix} U_0 &\ U_1 &\ \ldots &\ U_{N} \end{pmatrix}\) is a matrix containing a sequence of inputs, and \(W = \begin{pmatrix} W_0 &\ W_2 &\ \ldots &\ W_{N} \end{pmatrix}\) contains (noisy) meauserements of the correspondent outputs of the system, while \(Q = U^\bot\) has columns spanning the null space of \(U\).


==> TeX/Text/Simulations/QP.tex <==
Consider QPs as described in \Cref{ex:QP}
\begin{equation}
	\minimize_{x\in\R^n}\ \tfrac12 \innprod{Qx}{x} + \innprod{q}{x} + \delta_{C}(Ax)
\end{equation}
where \(Q\in\R^{n\times n}\) is symmetric and positive definite, \(q\in\R^n\), \(A\in\R^{m\times n}\), while \(C = \set{z\in\R^m}[z\leq b]\) with \(b\in\R^m\).
In order to specialize \Cref{alg:NAMA} to this case we simply need to evaluate the alternating minimization steps: by elementary manipulations we see that
\begin{align*}
	x(y)
&=
	\argmin_{x\in\R^n}\set{\tfrac12 \innprod{Qx}{x} + \innprod{q}{x} + \innprod{y}{Ax}}
\\
&=
	-Q^{-1}(\trans{A}y + q).
\end{align*}
Each \(x\)-step then requires a product by \(\trans{A}\) and \(Q^{-1}\).
In implementing \Cref{alg:NAMA}, we perform the latter using direct methods, \ie storing the Cholesky factorization of \(Q\). 
Alternatively one can use iterative methods for sparse, large scale problems, at the price of computing \(x(y)\) inexactly.

Furthermore
\begin{align*}
	z_\gamma(y)
&=
	\argmin_{z\in\R^m}\set{\delta_{\geq 0}(z) + \innprod{y}{Ax(y) + z - b} + \tfrac{\gamma}2\|Ax(y) + z - b\|^2}
\\
&=
	\argmin_{z\in\R^m}\set{\delta_{\geq 0}(z) + \tfrac{\gamma}2\|\gamma^{-1}y + Ax(y) + z - b\|^2}
\\
&=
	\proj_{\R^m_+}(\gamma^{-1} + Ax(y) - b),
\end{align*}
therefore \(z\)-steps only involve one product by \(A\) and a projection onto \(\R^m_+\).

We performed experiments using data \cite{ferreau2014online} from model predictive control (MPC) applications. We compared our proposed \Cref{alg:NAMA} with fast AMM, qpOASES 3.2.0 (active set method), the commercial QP solvers MOSEK 7.1 (interior point method) and TOMLAB/CPLEX 8.2 \hl{(what type of method is this?)}.
All solvers were run with default options, while \Cref{alg:NAMA} and fast AMM were stopped as soon as \(\|R_\gamma(y^k)\|_\infty \leq 10^{-8}\), \ie, when primal feasibility was satisfied up to a given tolerance.
For fairness, we only report the results on the problems for which the solution is not the unconstrained one: for each instance, we checked whether the origin is dual optimal, and skipped the problem when this was the case.
In fact, \Cref{alg:NAMA} and AMM in this case terminate at the first iteration when initialized at the origin, therefore any time comparison would simply measure preprocessing times.

%\Cref{tbl:QPdata} summarizes the parameters of the considered datasets, while the performance of the algorithms is illustrated in \Cref{fig:QPperf1}.

\begin{figure}
%	\input{TeX/Tikz/QP_random_fpr}
	\input{TeX/Tikz/QP_random_error}
	\caption{Convergence of \algacronym\ in a randomly generated QP. The vertical axis shows \(\|x^k-x_\star\|_\infty/\|x_\star\|_\infty\). In this experiment \(n=500, m=3n\), while \(Q\) and \(A\) were chosen so as to have \(10\%\) of nonzero normally distributed coefficients. The problem was generated starting from a known solution \(x_\star\) at which \(m/5\) constraints are active.}
\end{figure}

\begin{figure}
%\begin{minipage}{0.45\textwidth}
%	\input{TeX/Tikz/diesel_perf_cpu_time}
%\end{minipage}\hspace{1cm}
%\begin{minipage}{0.45\textwidth}
	\input{TeX/Tikz/chain80w_perf_cpu_time}
%\end{minipage}
\caption{Performance profiles of the CPU time (logarithmic scale) relative to the \texttt{chain80w} problem. While fast AMM performs poorly, \algacronym\ outperforms, in most of the cases, state of the art (and even commercial) QP solvers.}
\end{figure}
